Stop the Spread: A Contextual Integrity Perspective on the Appropriateness of COVID-19 Vaccination Certificates

We present an empirical study exploring how privacy influences the acceptance of vaccination certificate (VC) deployments across different realistic usage scenarios. The study employed the privacy framework of Contextual Integrity, which has been shown to be particularly effective in capturing people's privacy expectations across different contexts. We use a vignette methodology, where we selectively manipulate salient contextual parameters to learn whether and how they affect people's attitudes towards VCs. We surveyed 890 participants from a demographically-stratified sample of the US population to gauge the acceptance and overall attitudes towards possible VC deployments to enforce vaccination mandates and the different information flows VCs might entail. Analysis of results collected as part of this study is used to derive general normative observations about different possible VC practices and to provide guidance for the possible deployments of VCs in different contexts.

==> clmm_table1.tex <==
\begin{table*}[htb!]
\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{llllp{5em}}
                  %S[table-format = 1.2] 
                  %S[table-format = 1.2]
                  %S[table-format = 1.2]
                  %S[table-format = 1.3]
\toprule
Factors                  & \text{Est.} & \text{Std. Err} &Z & p\\ \midrule
%Intercept                  & -1.79965 & 0.60789 & -2.96  & 0.003072\twoS  \\ \hline
\multicolumn{5}{c}{Recipient: baseline=outdoor events}                 \\ 
\toprule
personal care          & 0.2265  & 0.3438  &   0.6589 & 0.5099592       \\ %\hline
worship                & 0.6411  & 0.3443  &   1.8617 & 0.04967418\oneS \\ %\hline
government Building         & 0.4463  & 0.3421   &  1.3044 & 0.1920930       \\ %\hline
apartment             & 1.2945 &  0.3446  &   3.7568 & 0.00011484\threeS\\ %\hline
eatery      & -0.1622 &  0.3553 &   -0.4589 & 0.6463340\\ %\hline
store         &  0.9848  & 0.3631  &   2.7120 & 0.00547035\twoS\\ %\hline
public transportation      &  0.3538 &  0.3393   &  1.0427 & 0.2971  \\ %\hline
gym        &  0.3293 &  0.3516   &  -0.9367 & 0.3489150\\ %\hline
entertainment       & 0.3410  & 0.3494 & 0.9758   & 0.3291871\\ %\hline
hotel      & 0.0888   & 0.3543 & 0.2506   & 0.8021       \\ %\hline
school           & -0.7414  & 0.3514 & -2.0196  & 0.03040020\oneS\\ %\hline
workplace    & 0.1652  & 0.3573 & 0.4596  & 0.6458\\ %\hline
assisted living facilities   & -1.7444  & 0.3687 & -4.7308  & .00000127\threeS\\ %\hline
hospitals & -0.2197  & 0.3539 & -0.6207  & 0.5348\\ %\hline
airline companies & -0.9421  & 0.3565  & -2.6428  & 0.00592741\twoS  \\ %\hline
cruise companies & -1.1023  & 0.3599  & -3.0630  & 0.00197805\twoS  \\ %\hline
Taxi/ridesharing drivers & 0.0116  & 0.3405  & 0.0340  & 0.9729  \\ %\hline
Taxi/ridesharing companies      & 0.0279  & 0.3479  & 0.0801  & 0.9361 \\ %\hline
large indoor event organizers & -0.6087  & 0.3474  & -1.7521  & 0.08068622\oneS  \\ %\hline
long-distance trains or buses      & -0.547  & 0.3472  & -1.5754  & 0.1151  \\ 
\bottomrule
\end{tabular}
}\caption{place holder}\label{tab:clmm}
\end{table*}

%\end{table}
\begin{comment}
\hline
\multicolumn{5}{c}{Likely: baseline=Less likely}                \\ %\hline
\toprule
about the same             & -3.5247 &  0.1970  & -17.8884 & 0.00000000000000022\threeS \\ %\hline
more likely                & -5.1914 &  0.2430  & -21.3635 & 0.00000000000000022\threeS \\ \hline
\multicolumn{5}{c}{Political: baseline=Conservative}      \\ %\hline        
\toprule
very conservative     & 0.9736 &  0.5190 &   1.8761 & 0.21140699  \\ %\hline
moderate              &  -0.6276 &   0.3101  &  -2.0239 & 0.04373492\oneS \\ %\hline
liberal               & -2.0039  & 0.2995   & -6.6920 & 0.00000012162\threeS \\ %\hline
very liberal          & 2.2414   & 0.3444   &-6.5077  & 0.00000020089\threeS \\ \hline
\multicolumn{5}{c}{Frequency}                      \\ 
\toprule
Frequency             & 0.0956 &  0.0426  &   2.2421 & 0.01647390\oneS \\ \hline
\multicolumn{5}{c}{Vaccinated: baseline=Prefer not to say}                           \\ %\hline
\toprule
Yes                   & -1.850 & 0.593 & -3.121 & 0.0018\twoS \\ %\hline
No                   & 0.460  & 0.608 & 0.759  & 0.4498\\ 
\end{comment}

==> clmm_table2_old.tex <==
%\begin{table}[htb!]
%\centering
\begin{table*}[h]

\resizebox{0.6\textwidth}{!}{
\begin{tabular}{llllp{5em}}
%\begin{tabular}{l S[table-format=2]S[table-format=2]S[table-format=2]S[table-format=2]}
%\bottomrule
\textbf{Factors}                  & \textbf{Est.} & \textbf{Std. Err} &\textbf{Z} & \textbf{$p$-value}\\ \bottomrule
%Intercept                  & -1.79965 & 0.60789 & -2.96  & 0.003072\twoS  \\%\hline
\multicolumn{5}{c}{\cellcolor{gray!20} \textbf{Sender}: baseline=customs and border control }                 \\ %\hline
\toprule
stores and restaurants                & 0.3526  & 0.1053  &  3.3476 & 0.00081508\threeS\\
recreational services or facilities & 0.4295  & 0.1058  &  4.0591 & 0.000049265\threeS\\%\hline
long-distance transportation        & 0.1446  & 0.1029  & 1.4060 & 0.15972230\\
public transportation operators     & 0.4104  & 0.1085  & 3.7833 & 0.00015474\threeS\\
rideshare and taxi companies       & 0.5943   & 0.1047  & 5.6749 & 0.000000013875\threeS\\
cruise companies         &  0.1940  & 0.1059 & 1.8316 & 0.06700569\\
large event organizers   & 0.3004 & 0.1083 & 2.7737 & 0.00554226\twoS\\%\hline
places of worship        & 0.4554 & 0.1094 & 4.1614 & 0.000031627\threeS\\
workplaces               & 0.2585  &   0.1087  &  2.3786 & 0.01737735\oneS\\
residential and real estate management & 0.5091 & 0.1097 & 4.6408 & 0.0000034707\threeS\\%\hline
schools                        & 0.3333  & 0.1076 &  3.0964 & 0.00195912\twoS\\
hospitals and assisted living facilities & 0.1423 & 0.1061 & 1.3402 & 0.18018126\\
government buildings           & 0.0360 & 0.1044 & 0.3449 & 0.73014683\\ %\hline
\bottomrule
\multicolumn{5}{c}{\cellcolor{gray!20} \textbf{Recipient}: baseline=public health protection agencies}                \\ %\hline
\toprule
local government             & 0.9632 & 0.0678 & 14.2105 &  2.2e-16\threeS\\%0.00000000000000022\threeS \\%\hline
federal government           & 0.9435 &  0.0678 & 13.9070 &  2.2e-16\threeS\\%0.00000000000000022\threeS \\%\hline
non profit organization      & 2.1072  & 0.0644 & 32.7192 & 2.2e-16\threeS\\% 0.00000000000000022\threeS \\%\hline
health insurer               & 2.3357  & 0.0655 & 35.6664 & 2.2e-16\threeS\\% \threeS \\%\hline
technology company           & 4.0112 & 0.0734 & 54.6408 & 2.2e-16\threeS\\%\threeS \\%\hline
business partners            & 3.7886 &  0.0718  &  52.7762 & 2.2e-16\threeS\\%\threeS \\%\hline
advertising and marketing partners & 4.5749 &  0.0782  &  58.5273 & 2.2e-16\threeS\\ \bottomrule%\hline%\threeS \\ 
\multicolumn{5}{c}{\cellcolor{gray!20} \textbf{Attribute}: baseline=vaccination certificate information}      \\ %\hline      
\toprule
location and time     & -0.0226  & 0.0410  &  -0.5520 & 0.5809257 \\ 
\bottomrule
\multicolumn{5}{c}{\cellcolor{gray!20} \textbf{Transmission Principle}: baseline=public health purposes}                           \\ %\hline
\toprule
other purposes                   &0.4224 & 0.0410 & 10.3004 & 2.2e-16\threeS\\%0.00000000000000022\\ 
\bottomrule
%
\end{tabular}}
\caption{Cumulative Linear Mixed Model Regression. A positive coefficient  (estimate) shows participants' decreased acceptance}\label{tab:clmm_tbl2}
\end{table*}


==> entities.tex <==
\begin{table*}
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{l|l|r|r}
%\toprule
 theme & description & mentions  & overall \%\\
\midrule
authoritative & trust the government or authority & 171 & 25\% \\
health & trust expertise, knowledge and/or experience in public health & 119 & 17.7\% \\

no vested interest & do not trust private businesses or entities that can profit from making VCs & 117 & 17.4\% \\

proficient & trust entities that have resources, money, technology or professionals to develop VCs & 81 & 12\%\\
id-making experience & trust entities that have existing infrastructures to make IDs that cannot be easily counterfeited & 51 & 7.6\%\\
security & trust entities that can keep their information safe or distrust otherwise & 54 & 8\%\\
standardized  & trust entities that can produce nationally standardized VCs     & 46 & 6.8\%\\

bipartisan  &   trust only the state or only the federal & 45 & 6.7\%\\

impartial & trust entities that are free from biases & 41 & 6.1\%\\
privacy & trust entities that can keep information private or distrust otherwise & 38 & 5.6\%\\

responsible  & trust entities that have the public's safety and interest in mind  & 35 & 5.2\%\\
%no profit & do not trust private businesses or entities that can profit from making VCs & 65 & 10\% \\

international  & trust entities that develop VCs recognized internationally & 26 & 3.9\%\\
accountable  &   trust VCs developed by entities that can be held accountable & 25 & 3.7\%\\

\bottomrule
 %   experience_id \\
\end{tabular}
}\caption{List of themes mentioned by least 20 participants and their respective descriptions and percentages (out of 674)}~\label{tab:entities}
\end{table*}

==> vignettes.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|l}
Sender            & Recipient                          & Transmission Principle                                \\ 
\toprule
Passengers        & airline companies                   & take an international flight                          \\ \hline
Foreign travelers & \multirow{2}*{customs and border controls}          & enter the United States         \\ 
US nationals      &         & enter a foreign country                               \\ \hline
Students          & \multirow{2}*{schools (K-12 and higher education)} & return to in-person learning    \\ 
Teachers          &         & return a in-person learning                           \\ \hline
\multirow{3}*{Job applicants}   & \multirow{3}*{employers }                          & be considered for a job                               \\ 
   &                          & be considered for a job in hospitals                  \\ 
   &                           & be considered for a job in assisted living facilities \\ \hline
Potential renters & building management                 & rent an apartment                                     \\
\bottomrule
\end{tabular}%
}
\caption{Caption goes here}\label{tab:vignettes}
\end{table}
